Counting Butterflies in Fully Dynamic Bipartite Graph Streams

A bipartite graph extensively models relationships between real-world entities of two different types, such as user-product data in e-commerce. Such graph data are inherently becoming more and more streaming, entailing continuous insertions and deletions of edges. A butterfly (i.e., 2x2 bi-clique) is the smallest non-trivial cohesive structure that plays a crucial role. Counting such butterfly patterns in streaming bipartite graphs is a core problem in applications such as dense subgraph discovery and anomaly detection. Yet, existing approximate solutions consider insert-only streams and, thus, achieve very low accuracy in fully dynamic bipartite graph streams that involve both insertions and deletions of edges. Adapting them to consider deletions is not trivial either, because different sampling schemes and new accuracy analyses are required. In this paper, we propose Abacus, a novel approximate algorithm that counts butterflies in the presence of both insertions and deletions by utilizing sampling. We prove that Abacus always delivers unbiased estimates of low variance. Furthermore, we extend Abacus and devise a parallel mini-batch variant, namely, Parabacus, which counts butterflies in parallel. Parabacus counts butterflies in a load-balanced manner using versioned samples, which results in significant speedup and is thus ideal for critical applications in the streaming environment. We evaluate Abacus/Parabacus using a diverse set of real bipartite graphs and assess its performance in terms of accuracy, throughput, and speedup. The results indicate that our proposal is the first capable of efficiently providing accurate butterfly counts in the most generic setting, i.e., a fully dynamic graph streaming environment that entails both insertions and deletions. It does so without sacrificing throughput and even improving it with the parallel version.

==> architecture.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Architecture}
\label{sec:architecture}
%%%%%%%%%%%%%%%%%%%%%%%%

Let us now elaborate on \abacus's architecture\jorge{Architecture? ISn't Abacus and algorithm?}, our mini-batch streaming algorithm for counting butterflies in a fully dynamic bipartite graph stream under infinite window semantics. 
First, we provide \abacus's building blocks in the centralized setting. 
Then, we detail on which of these components parallelize for leveraging all the available threads %of a multicore %shared-memory machine.
to maximize throughput. 

\jorge{I am really confused by this section. You say that you first define building block of Abacus and then you explain which of these blocks you extend to achieve parallization, right? My confusion then comes from grasping the goal of this entire section: I would move the building block to Section 4 and the discussion on how you leverage such building blocks for parallization into Section 5.}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.4\textwidth]{figures/abacus-architecture.pdf}
  \caption{\abacus's main architecture.}
  \makis{highlight the heavy-hitter tracking in the architecture.}
  \label{fig:architecture-abacus} 
\end{figure}




%%% --------------------------------
\subsection{Centralized Setting}
\label{subsec:centralized-architecture}

Here, we give the general workflow of \abacus, and essentially present its core components\jorge{What do you discuss in the next section then?}. 
Figure~\ref{fig:architecture-abacus} illustrates the main architecture\jorge{dataflow?} of \abacus, i.e., all the essential building blocks that constitute our solution. 
\abacus ingests a fully dynamic graph stream, which is a series of element sequences (i.e., minibatches) either fixed \textcolor{red}{or varying} size. 
Recall that the stream elements in each minibatch consist of an edge $\{u, v\}$ and a sign $\delta$ that signifies an insertion or a deletion. 
\abacus processes each minibatch as soon as it arrives, and afterward, it evicts it from the main memory. 
Note that minibathes may be quite large in size (possibly in the order of GB or more). 
% Thus, \abacus relies on parallelism, which is common wisdom for utilizing all the available threads in a shared-memory multicore machine to achieve maximum throughput when counting butterflies. 

\abacus continuously observes and receives a potentially infinite sequence of minibatches of a fully dynamic bipartite graph stream. 
It always maintains a uniform random sample, $\mathcal{S}$\jorge{where is S in the Figure?}, using the Random Pairing (RP)~\cite{vldbj08-gemulla} sampling scheme, which works for streams that contain both edge insertions and deletions. 
Note that in the centralized setting, sampling and updating butterfly counts are conducted using only one thread. 
Therefore, the partition function, $\mathcal{P}$, does not split the edges inside a minibatch to multiple threads for processing, i.e.,~it is in a sense dummy. 
Afterward, \abacus uses the existing sample, $\mathcal{S}$ when invoking the $\mathtt{UpdateBC}$ function\jorge{what is BC?} that updates the butterfly estimates such that they always stay unbiased and retain low variance. 
Then, \abacus invokes $\mathtt{UpdateS}$, which actually applies the sampling scheme's decisions for a specific minibatch regarding which edges from $\mathcal{S}$ should be inserted to or deleted from $\mathcal{S}$. 
Note that in its centralized version \abacus does not have to merge partial butterfly estimates of multiple threads into a global and the corresponding local (per vertex) counts. 
Therefore, the merge function, $\mathcal{M}$, is a dummy\jorge{identity? In fact, I think that P() and M() are introduced by PARABACUS, so why to have them from now on?} here. 
In the streaming scenario, it is really important to have both the global and local counts always readily available; especially for applications such as anomaly detection and dense subgraph detection. 
% (see~\ref{subsec:anomaly-detection, subsec:dense-subgraph-detection}). 
Towards this end, \abacus should achieve the maximum throughput possible while using limited and small memory at the same time. 

% \begin{enumerate}
    % \item elements (edge + sign) of the graph stream are revealed in a series of element sequences, i.e.,~mini-batches.
    
    % \item since we are dealing with fully dynamic bipartite graph streams, the mini-batches may have both edge insertions and deletions. 
    
    % \item infinite window semantics, i.e., \abacus draws samples (using RP~\cite{vldbj08-gemulla}) from all the elements received.
    
    % \item We provide complexity analysis of \abacus for both time and space, in the centralized setting.
% \end{enumerate}



%%% --------------------------------
\subsection{Parallel Setting}
\label{subsec:parallel-architecture}

\abacus relies on parallelism for utilizing all the available threads in a shared-memory multicore machine to achieve maximum throughput when counting butterflies. 
Let us now elaborate on which of \abacus components can and is beneficial to be parallelized for increasing performance in the mini-batch streaming scenario. 

The parallel version of \abacus, namely, \parabacus, strives to 
fully process each minibatch in parallel. 
\parabacus conducts the sampling from every single minibatch in parallel using a novel scheme that is a combination of Random Pairing (RP)~\cite{vldbj08-gemulla}, which produces uniform random samples in fully dynamic streams, and the method presented in~\cite{arxiv19-tirthapura, toms18-sanders}, which samples in parallel and without replacement from insertion-only streams. 
In a nutshell, it is favorable to maintain a uniform random sample and in parallel, so that we produce unbiased butterfly estimates and retain high throughput. 
Note that we use infinite window semantics to conduct the butterfly counting over an incoming fully dynamic graph stream. 
%%%
\makis{Do the methods~\cite{arxiv19-tirthapura} and~\cite{toms18-sanders} partition the stream beforehand to do the sampling? read them carefully again. In essence, is the sampling processing heavily and qualitatively affected by the partitioning method?} 
%%% partitioning
In \parabacus, we follow the data-parallel paradigm that partitions the edges in each minibatch into disjoint sets and distributed these sets into distinct processing units (i.e.,~threads). 
Each thread retains its independent data structures 
\makis{check the persistent data structures~\cite{tods22-ke}} 
for conducting the butterfly counting and deriving the final merged global and local count(s). 
At the same time, we used a shared-memory data structure that maintains the bipartite graph sample, $\mathcal{S}$, which is  simultaneously accessed by different threads. 
% \makis{When will different threads apply the actual sample update? check persistent data structures that have versions~\cite{tods22-ke}. Maybe the shared data structure for the sample can/should be a persistent data structure.}  

%Note that t
The partitioning function, $\mathcal{P}$, plays a crucial role as it directly affects the butterfly estimate update process, i.e.,~$\mathtt{UpdateBC}$. 
More specifically, efficient \textit{load-balancing} is required for avoiding stragglers %processing units 
and resource under-utilization.  
\parabacus devises a novel partitioning scheme that is based on \textit{heavy hitter tracking} so that it assigns edges and tasks to threads using the distribution of vertex degrees.   
Ultimately, \parabacus partitions the graph stream such that it achieves a balanced execution. 
\makis{does partitioning affect the sampling?} 
Furthermore, the merging function, $\mathcal{M}$, which combines the partial butterfly count estimates of each thread into the final one, should be associative and communicative (e.g.,~sum and average) to be robust and independent of the sequence that the partial counts are updated. 
Finally, we prove that \abacus and our parallel full-fledged version, \parabacus, maintain unbiased butterfly count estimates of the low variance in parallel, and our algorithm is work-efficient and uses small space. 

In the sequel, we first present the specifics of \abacus, our centralized solution, and then elaborate on the details of \parabacus, our final parallel efficient method for estimating butterflies counts. 



% \begin{enumerate}
    % \item elements (edge + sign) of the graph stream are revealed in a series of element sequences, i.e.,~mini-batches. (\textcolor{red}{same as in the centralized setting}). 
    % Since we are dealing with fully dynamic bipartite graph streams, the mini-batches may have both edge insertions and deletions. 
    
    % \item infinite window semantics, i.e., \abacus draws samples (using RP~\cite{vldbj08-gemulla}) from all the elements received. 
    % \textcolor{blue}{The core aspect in this subsection is to highlight which building blocks we parallelized, with which existing algorithms, and why...}
    
    % \item We provide complexity analysis of \abacus for both time and space, in the parallel setting \textcolor{blue}{using the work-depth model}. 
    % This work strives for \textit{parallel work-efficiency} except for small memory footprint.
    
    % \item Stress that \textit{partitioning} is quite important not only for fast parallel sampling but mainly for a \textit{load-balanced} parallel execution. 
    
    % \item Note that the \textit{merging function} should be associative and blah blah, and allowing for in-parallel evaluation. 
    % Its final output should be the same irrespective of the sequence of the operations.  
% \end{enumerate}



\makis{should have figure 1. Assume centralized setting. That figure won't have p and m. merge 3 with abacus section.}
